On the Connection Between MPNN and Graph Transformer

Graph Transformer (GT) recently has emerged as a new paradigm of graph learning algorithms, outperforming the previously popular Message Passing Neural Network (MPNN) on multiple benchmarks. Previous work (Kim et al., 2022) shows that with proper position embedding, GT can approximate MPNN arbitrarily well, implying that GT is at least as powerful as MPNN. In this paper, we study the inverse connection and show that MPNN with virtual node (VN), a commonly used heuristic with little theoretical understanding, is powerful enough to arbitrarily approximate the self-attention layer of GT. In particular, we first show that if we consider one type of linear transformer, the so-called Performer/Linear Transformer (Choromanski et al., 2020; Katharopoulos et al., 2020), then MPNN + VN with only O(1) depth and O(1) width can approximate a self-attention layer in Performer/Linear Transformer. Next, via a connection between MPNN + VN and DeepSets, we prove the MPNN + VN with O(n^d) width and O(1) depth can approximate the self-attention layer arbitrarily well, where d is the input feature dimension. Lastly, under some assumptions, we provide an explicit construction of MPNN + VN with O(1) width and O(n) depth approximating the self-attention layer in GT arbitrarily well. On the empirical side, we demonstrate that 1) MPNN + VN is a surprisingly strong baseline, outperforming GT on the recently proposed Long Range Graph Benchmark (LRGB) dataset, 2) our MPNN + VN improves over early implementation on a wide range of OGB datasets and 3) MPNN + VN outperforms Linear Transformer and MPNN on the climate modeling task.

==> climate.tex <==
\vspace{-5pt}
\subsection{Forecasting Sea Surface Temperature} \label{sec:climate}

In this experiment, we apply our MPNN + VN model to forecast sea surface temperature (SST). We are particularly interested in the empirical comparison between MPNN + VN and Linear Transformer \citep{katharopoulos-et-al-2020} as according to \Cref{sec:shallow-narrow-attention}, MPNN + VN theoretically can approximate Linear Transformer.

In particular, from the DOISST data proposed by \citep{ImprovementsoftheDailyOptimumInterpolationSeaSurfaceTemperatureDOISSTVersion21}, we construct a dataset of daily SST in the Pacific Ocean from 1982 to 2021, in the region of longitudes from $180.125^\circ\text{E}$ to $269.875^\circ\text{E}$ and latitudes from $-14.875^\circ\text{N}$ to $14.875^\circ\text{N}$. Following the procedure from \citep{de2018deep,deBezenac2019} and \citet{wang2022metalearning}, we divide the region into 11 batches of equal size with 30 longitudes and 30 latitudes at 0.5$^\circ$-degree resolution, that can be represented as a graph of 900 nodes. 
% in which we connect each node to its nearest 8 neighbors. 
The tasks are to predict the next 4 weeks, 2 weeks and 1 week of SST at each location, given 6 weeks of historical data. We train on data from years 1982--2018, validate on data from 2019 and test on data from 2020--2021. The number of training, validation, and testing examples are roughly 150K, 3K, and 7K. See details of dataset construction, model architectures, and training scheme in \Cref{appendix:climate}. %\chen{add somewhere about the data size as people will wonder whether the small margin is statistically significant}



We compare our model to other baselines including TF-Net \cite{Rui2020}, a SOTA method for spatiotemporal forecasting, Linear Transformer \citep{katharopoulos-et-al-2020,wang2020linformer} with Laplacian positional encoding (LapPE), and Multilayer Perceptron (MLP). We use Mean Square Error (MSE) as the metric and report the errors on the test set, shown in the \Cref{tab:climate}. 
We observe that the virtual node (VN) alone improves upon MPNN by $3.8\%$, $6.6\%$ and $4.5\%$ in 4-, 2- and 1-week settings, respectively. Furthermore, aligned with our theory in \Cref{sec:shallow-narrow-attention}, MPNN + VN indeed achieves comparable results with Linear Transformer and outperforms it by a margin of $0.4\%$, $2.8\%$ and $4.3\%$ in 4-, 2- and 1-week settings, respectively.

%Furthermore, aligned with our theory in \Cref{sec:shallow-narrow-attention}, MPNN + VN + LapPE indeed achieves comparable results with Linear Transformer and outperforms it by a margin of $0.4\%$, $3.7\%$ and $6\%$ in 4-, 2- and 1-week settings, respectively. The VN alone can help MPNN to outperform Linear Transformer as well, but with slightly smaller margins.

